TRACE: Discovering Task-Specific Parameter via Adaptation-Aware Probing for Continual Fine-Tuning

In real-world deployment, LLMs are often adapted continually across tasks to keep LLMs up-to-date in production, where new fine-tuning should preserve previously learned skills. However, indiscriminately mixing tasks can dilute task specialization, while sequential fine-tuning (full-parameter or low rank adaptation) often causes catastrophic forgetting due to destructive overwriting. Replay-based continual tuning and maintaining separate task-specific adapters can mitigate forgetting, but introduce additional compute, storage, and management overhead. Recognizing the redundancy of LLM parameters for any single task, we reframe continual task adaptation as task-specific parameter discovery via adaptation-aware probing: a short warm-start probe exposes a task's adaptation trace, enabling us to identify and isolate the small subset of parameters essential for each task to mitigate catastrophic forgetting. Building on this view, we introduce TRACE, a novel approach for discovering Task-specific paRameters via Adaptation-aware probing for Continual finE-tuning. We perform a short warm-start fine-tune to derive task-specific core parameters by comparing the warm-started and pre-trained models. Core parameters are identified via two strategies: importance scoring (L$_2$ norm and Fisher Information) and specificity analysis (cosine similarity of parameter updates). In continual fine-tuning settings, only the active task's core parameters are updated while others remain frozen, preserving prior knowledge. We conduct extensive experiments across multiple standard benchmarks to demonstrate the superior performance of our proposed method. Additionally, we validate the generalization of our method through a cross-model and scale transferability study, demonstrating a "small-to-large" paradigm that guides the fine-tuning of large-scale models under resource constraints.

==> preliminary.tex <==
\section{Preliminary Study}
In this section, we introduce the foundational concepts of LLMs and SFT, which serve as the basis for multi-task adaptation strategy.

%\subsection{Large Language Models}
\noindent \textbf{Large Language Models.}
LLMs define a conditional distribution over textual outputs $y = (y_1, \dots, y_L)$ given an input prompt $x = (x_1, \dots, x_M)$. Let $f_\theta(y \mid x)$ denote such distribution, where $\theta$ represents the model parameters. In the autoregressive setting, $f_\theta$ decomposes the output probability as:
\begin{equation}
f_\theta(y \mid x) = \prod_{l=1}^L f_\theta(y_l \mid x, y_{<l}),
%\tag{1}
\end{equation}
where $y_{<l} = (y_1, \dots, y_{l-1})$ represents the previously generated tokens. Typically, $f_\theta$ is instantiated using a multi-layer Transformer \cite{vaswani2017attention} decoder trained on massive unlabeled corpora.

Through pretraining, the model acquires general-purpose capabilities, but domain-specific adaptation is often required for specialized applications (\textit{e.g.}, biomedical QA or code synthesis). This motivates the need for SFT.

%\subsection{Supervised Fine-Tuning}
\noindent \textbf{Supervised Fine-Tuning.}
SFT is a standard approach to adapt pretrained LLMs to specific downstream tasks. It leverages instruction-response pairs $(x, y)$ drawn from a labeled dataset $\mathcal{D} = \{(x_i, y_i)\}_{i=1}^N$. The objective is to optimize the model parameters $\theta$ to maximize the likelihood of the desired outputs under the data distribution:
\begin{equation}
\mathcal{L}_{\text{SFT}}(\theta) = \mathbb{E}_{(x, y) \sim \mathcal{D}} \left[ - \log f_\theta(y \mid x) \right].
%\tag{2}
\end{equation}

This loss is typically implemented as token-level cross-entropy. Notably, SFT assumes a fixed data distribution and does not account for potential task interference when training sequentially on multiple domains.
 

==> theory.tex <==
\section{Theoretical Analysis}
In this section, we provide formal theoretical justification for TRACE by addressing two fundamental questions: \textit{(Q1) Does restricting gradient updates to a small core parameter set $\mathcal{C}_k$ compromise the optimization efficiency on the current task?} \textit{(Q2) How does the structural separation of core parameter sets across tasks control catastrophic forgetting, and can TRACE scale to long task sequences?} We answer these questions through two theorems, a proposition, and a corollary, with all formal proofs deferred to \textbf{Appendix}~\ref{proof}.

\noindent\textbf{Notation.} Let $\mathcal{L}_k(\theta)$ denote the loss on task $T_k$, $d$ the total number of parameters, and $\mathcal{C}_k \subseteq [d]$ the core parameter set for task $T_k$ with $|\mathcal{C}_k| = \rho d$ where $\rho = r/100$. We write $\nabla_{\mathcal{C}_k}\mathcal{L}_k$ for the gradient restricted to coordinates in $\mathcal{C}_k$.

\begin{definition}[Gradient Energy Ratio]
\label{def:ger}
For task $T_k$ with core set $\mathcal{C}_k$, the \emph{gradient energy ratio} at $\theta$ is defined as:
\begin{equation}
    \gamma_k(\mathcal{C}_k, \theta) := \frac{\|\nabla_{\mathcal{C}_k} \mathcal{L}_k(\theta)\|_2^2}{\|\nabla \mathcal{L}_k(\theta)\|_2^2},
\end{equation}
which measures the fraction of the full gradient's energy captured by $\mathcal{C}_k$.
\end{definition}

\begin{theorem}[Optimization Efficiency of Core Parameter Training]
\label{thm_opt}
Assume $\mathcal{L}_k$ is $L$-smooth. With learning rate $\eta \leq 1/L$, a single gradient descent step restricted to $\mathcal{C}_k$ achieves:
\begin{equation}
    \mathcal{L}_k(\theta') \leq \mathcal{L}_k(\theta) - \frac{\eta}{2}\|\nabla \mathcal{L}_k(\theta)\|_2^2 \cdot \gamma_k(\mathcal{C}_k, \theta),
\end{equation}
where $\theta' = \theta - \eta \cdot \nabla_{\mathcal{C}_k}\mathcal{L}_k(\theta)$. Consequently, the per-step loss reduction of core-only training is at least a $\gamma_k$-fraction of that achieved by full-parameter training.
\end{theorem}

Theorem~\ref{thm_opt} shows that the key to effective selective training is achieving $\gamma_k \approx 1$. We further show (Proposition~\ref{prop:strategy} in \textbf{Appendix}~\ref{proof}) that both TRACE strategies are designed to maximize $\gamma_k$: the L2-Fisher score ranks parameters by a combination of accumulated and instantaneous gradient energy, while the cosine similarity score prioritizes coordinates whose gradient energy is concentrated on the current task. Together, they ensure that restricting updates to a small core set incurs minimal optimization loss.

We now turn to the second question: how selective activation controls forgetting.

\begin{definition}[Core Set Overlap Ratio]
\label{def:overlap}
For two tasks $T_j$ and $T_k$, the \emph{core set overlap ratio} is:
\begin{equation}
    \omega_{j,k} := \frac{|\mathcal{C}_j \cap \mathcal{C}_k|}{|\mathcal{C}_j|},
\end{equation}
which measures the fraction of task $T_j$'s core parameters that are also activated during training on $T_k$.
\end{definition}

\begin{theorem}[Forgetting Bound via Core Set Overlap]
\label{thm_forget}
Assume $\mathcal{L}_j$ is $L$-smooth. After one gradient step on task $T_k$ with core set $\mathcal{C}_k$ and learning rate $\eta \leq 1/L$, the interference on a previous task $T_j$ satisfies:
\begin{equation}
\begin{aligned}
    \Delta \mathcal{L}_j^{\mathrm{interf}} &\leq \underbrace{\|\nabla_{\mathcal{C}_j \cap \mathcal{C}_k} \mathcal{L}_j\|_2 \cdot \eta \|\nabla_{\mathcal{C}_j \cap \mathcal{C}_k} \mathcal{L}_k\|_2}_{\text{(I) shared core interference}} \\
    &+ \underbrace{\|\nabla_{\mathcal{C}_k \setminus \mathcal{C}_j} \mathcal{L}_j\|_2 \cdot \eta \|\nabla_{\mathcal{C}_k \setminus \mathcal{C}_j} \mathcal{L}_k\|_2}_{\text{(II) non-core interference}} + O(\eta^2).
\end{aligned}
\end{equation}
Term~(I) is controlled by the overlap ratio $\omega_{j,k}$: when $\omega_{j,k} \to 0$, this term vanishes. Term~(II) is inherently small because $\mathcal{C}_k \setminus \mathcal{C}_j$ consists of parameters that are non-core for $T_j$, for which $\|\nabla_{\mathcal{C}_k \setminus \mathcal{C}_j} \mathcal{L}_j\|_2$ is small by the definition of core parameter selection.
\end{theorem}

Theorem~\ref{thm_forget} reveals that TRACE's forgetting is governed by the \emph{structural separation} between core sets, not merely by the act of freezing parameters. When different tasks activate distinct parameter subsets ($\omega_{j,k} \approx 0$), both interference terms become negligible.

Combining Theorems~\ref{thm_opt} and~\ref{thm_forget}, we further show (Corollary~\ref{cor:capacity} in \textbf{Appendix}~\ref{proof}) that increasing $\rho$ improves $\gamma_k$ but raises $\omega_{j,k}$, yielding an optimal sparsity $\rho^*$ that balances current-task learning against forgetting. This explains the empirical peak at $r\approx 5\%$ (Sec.~\ref{sec:r_sens}) and the scalability to long task sequences (Sec.~\ref{sec:longseq}).
